Why Don't You Clean Your Glasses? Perception Attacks with Dynamic Optical Perturbations

Camera-based autonomous systems that emulate human perception are increasingly being integrated into safety-critical platforms. Consequently, an established body of literature has emerged that explores adversarial attacks targeting the underlying machine learning models. Adapting adversarial attacks to the physical world is desirable for the attacker, as this removes the need to compromise digital systems. However, the real world poses challenges related to the "survivability" of adversarial manipulations given environmental noise in perception pipelines and the dynamicity of autonomous systems. In this paper, we take a sensor-first approach. We present EvilEye, a man-in-the-middle perception attack that leverages transparent displays to generate dynamic physical adversarial examples. EvilEye exploits the camera's optics to induce misclassifications under a variety of illumination conditions. To generate dynamic perturbations, we formalize the projection of a digital attack into the physical domain by modeling the transformation function of the captured image through the optical pipeline. Our extensive experiments show that EvilEye's generated adversarial perturbations are much more robust across varying environmental light conditions relative to existing physical perturbation frameworks, achieving a high attack success rate (ASR) while bypassing state-of-the-art physical adversarial detection frameworks. We demonstrate that the dynamic nature of EvilEye enables attackers to adapt adversarial examples across a variety of objects with a significantly higher ASR compared to state-of-the-art physical world attack frameworks. Finally, we discuss mitigation strategies against the EvilEye attack.

==> Sources/motivating.tex <==
\section{Motivating Example}
\label{sec:motivating}


As is shown in \autoref{fig:setup-diagram}, an autonomous driving vehicle is equipped with a camera sensor. The camera sensor continuously precepts the scene in front the vehicle. The video frames percepted by the camera sensor are sent to a traffic sign recognition module. The outputs of the recognition module controls what actions the vehicle needs to take (e.g., stop in front of a stop sign or slow down when a 55 speed limit sign is observed).

An adversary intended to attack this vehicle prepares a transparent displaying gadget (\autoref{fig:trans-display}) and install the gadget in front of the camera sensor. The adversary can remotely control the gadget to display adversarial perturbations. In this way, the normal operation of the vehicle is disturbed and possibly leads to catastrophic consequences such as crash.

Based on different level of knowledge the adversary has of the camera under attack, he needs to take different actions and the effectiveness of the attack also varies. Under a White box scenario, where the adversary has full knowledge about the recognition module, i.e., he has access to the architecture and weights of the model as well as the gradient information during the inference of a frame, he needs to prepare various pictures of the traffic sign to be attacked, and generate a universal adversarial perturbation (UAP) based these images. Under a black box setting, the adversary needs to utilize the transferability of adversarial examples, i.e., he needs to craft the UAP based on a different recognition model, and apply the UAP to the camera under attack. He can use a publically available traffic sign dataset to train a widely used image recognition model. He then crafts UAPs based on this model.

The attacker can dynamically change the displayed perturbation. This gives him the advantage of ...
